Disappearing frameworks explained

The web is the most prominent application platform globally, thanks to its vast user base. It started as a site platform in the 90s and morphed into an application one over time as interactive web applications became a reality. So-called single-page applications (SPAs) represent the current mainstream way of developing web applications but they come with their drawbacks. Although SPAs provide good developer experience, there is a cost for the users due to the underlying technical assumptions. Disappearing frameworks question these assumptions and provide a fresh start. The purpose of this short book is to give a quick introduction to disappearing frameworks and show their meaning as an emerging topic within the space of web application development.

==> 01-plan.tex <==
\textbf{A. Topic, shape, and authors}

\begin{enumerate}
    \item Topic and name of the work - Disappearing frameworks explained
    \item Who is doing and what - Juho Vepsäläinen will do everything
    \item How is the entity developed within the exercise defined - In this case the entity is a booklet. The target is to write ~20-40 page short book that delves into the topic of disappearing frameworks from the developer point of view. It is still an emerging research topic so it's possible I won't be able to complete the booklet fully but at least it should help me to understand the current research gaps that I can fill in my research.
    \item Who is the entity meant for? - The target is to reach advanced web developers with the work and help to popularize the ideas behind disappearing frameworks.
\end{enumerate}

\textbf{B. Target, background and justifications}

\begin{enumerate}
    \item Why this topic and target? How does it serve your own development? - The topic is at the heart of my research and I believe making it more visible to the public would help in making it more known in the community while motivating my research efforts further. I believe completing the booklet in a timely manner would further bolster my reputation as a book author as it is something I could publish through my own publishing company. A good option would be to develop a web portal around the content. In any case, writing about the topic in a popular manner is a good idea as it an be shaped to fit media.
    \item Shape of the exercise - In this case, the initial product of the work will be a pdf file that is then delivered to the course platform
    \item What kind of methods, tools or forms or work are used - I will use overleaf.com for writing. To keep it simple, I will rely on written references. Comments and interviews from the developer community would complement the booklet well and may be worth adding after there is an initial draft to show around.
    \item What kind of source material is used in the work - I will rely mainly on the references I have discovered during my research so far. I will also refer to a couple of published papers of my own. One challenge is that some of the information is available only in unpublished form so that will make sourcing slightly challenging.
    \item Is the target to share the outcome outside of the course (how, where, to whom) - Most likely it makes sense to share the first draft to the tool authors to try to attract quotes from them as that would increase the value of the booklet. After this round of feedback, it would likely make sense to publish it to the publish even using a "pay what you want" kind of model to keep it affordable while giving a chance to earn revenue.
\end{enumerate}

\textbf{Execution plan}

\begin{enumerate}
    \item What kind of phases does the work consist of and how to complete it before 22.5 - Given there are only three weeks to complete the work, it means I will have to move fairly fast. As a result, I've divided the work to three iterations target of each is to complete a full chapter. Likely the last chapter is shorter than the main ones meaning more focus can be given to editing during the last pass. To turn the booklet into a full book, most likely some of the topics discussed would have to become chapters of their own but in the scope of this work it is enough to cover the key topics in some detail.
\end{enumerate}

\begin{comment}
A. Tehtävän aihe, muoto ja tekijä(t)
● Mikä on tehtävän aihe ja työnimi/otsikko?
● Kuka tai ketkä ovat osallisia tehtävässä (millainen työnjako, osallistujien roolit?)
● Millaisen kokonaisuuden kehittämistehtävä muodostaa?
● Kenelle tuotos on suunnattu (yleisö/kohderyhmä)?
B. Tehtävän tavoite, tausta ja perustelut
● Miksi tämä aihe ja tavoite? Millä tavoin se palvelee omaa osaamistavoitteitasi?
● Tehtävän muoto? Valinta sen mukaan, mikä palvelee tavoitetta. Tulee olla palautettuna jossain
muodossa (tiedostona, linkkinä tms.) kurssialueelle 22.5. mennessä. Huom! Jos kyseessä on laajempi
yleistajuistamistehtävä johonkin tiettyyn tarkoitukseen kurssin ulkopuolella, voit tuoda alustalle
sopivan osan/vaiheen ja kuvata, miten työ jatkossa etenee.
● Millaisia menetelmiä, välineitä tai työmuotoja käytetään?
● Mitä lähdemateriaalia tehtävässä hyödynnetään (tiedepohjaisuus)?
● Onko tavoitteena jakaa tuotos kurssin ulkopuolella (miten, missä, kenelle)?
C. Toteuttamissuunnitelma
● Millaisista vaiheista tehtävä koostuu ja millaisin etapein työ valmistuu jaettavaksi 22.5. mennessä?
Jos parityö/ryhmäprojekti: työnjako (kuka tekee mitäkin)
\end{comment}

